Open World Classification with Adaptive Negative Samples

Open world classification is a task in natural language processing with key practical relevance and impact. Since the open or {\em unknown} category data only manifests in the inference phase, finding a model with a suitable decision boundary accommodating for the identification of known classes and discrimination of the open category is challenging. The performance of existing models is limited by the lack of effective open category data during the training stage or the lack of a good mechanism to learn appropriate decision boundaries. We propose an approach based on \underline{a}daptive \underline{n}egative \underline{s}amples (ANS) designed to generate effective synthetic open category samples in the training stage and without requiring any prior knowledge or external datasets. Empirically, we find a significant advantage in using auxiliary one-versus-rest binary classifiers, which effectively utilize the generated negative samples and avoid the complex threshold-seeking stage in previous works. Extensive experiments on three benchmark datasets show that ANS achieves significant improvements over state-of-the-art methods.

==> tabels/appdix_discuss_neg_banking.tex <==
\begin{table}[]
\begin{center}
\begin{sc}
   \scalebox{0.68}{
   \begin{tabular}{@{}lccccc@{}}
\toprule
\%                  & Methods                  & Acc   & F1    & F1-open & F1-known \\ \midrule
\multirow{4}{*}{25} & Baseline ($\lambda = 0$) & 43.54 & 50.83 & 41.40   & 51.33    \\
                    & \(+\) Gaussian Noise     & 71.37 & 67.02 & 77.55   & 66.46    \\
                    & \(+\) Projection         & 80.05 & 73.17 & 85.51   & 72.52    \\
                    & \(+\) Ascend (Ours)      & 80.11 & 73.35 & 85.57   & 72.71    \\ \cmidrule(l){2-6} 
\multirow{4}{*}{50} & Baseline ($\lambda = 0$) & 59.42 & 70.96 & 41.69   & 71.73    \\
                    & \(+\) Gaussian Noise     & 77.23 & 81.02 & 75.27   & 81.17    \\
                    & \(+\) Projection         & 82.00 & 83.04 & 82.28   & 83.06    \\
                    & \(+\) Ascend (Ours)      & 81.79 & 83.02 & 81.95   & 83.05    \\ \cmidrule(l){2-6} 
\multirow{4}{*}{75} & Baseline ($\lambda = 0$) & 67.26 & 73.99 & 64.30   & 74.12    \\
                    & \(+\) Gaussian Noise     & 81.49 & 86.80 & 64.88   & 87.17    \\
                    & \(+\) Projection         & 82.05 & 86.70 & 69.37   & 87.00    \\
                    & \(+\) Ascend (Ours)      & 82.16 & 86.68 & 69.70   & 86.98    \\ \cmidrule(l){2-6} 
\end{tabular}
% \begin{tabular}{llcccc}
% \hline
% \%                  & Methods                  & Acc   & F1    & F1-open & F1-known \\ \hline
% \multirow{4}{*}{25} & Baseline ($\lambda = 0$) & 43.54 & 50.83 & 41.4    & 51.33    \\
%                     & \(+\) Gaussian Noise     & 71.37 & 67.02 & 77.55   & 66.46    \\
%                     & \(+\) Projection         & 72.79 & 68.61 & 78.9    & 68.07    \\
%                     & \(+\) Ascend (Ours)      & 80.27 & 73.42 & 85.71   & 72.89    \\ \hline
% \multirow{4}{*}{50} & Baseline ($\lambda = 0$) & 59.42 & 70.96 & 41.69   & 71.73    \\
%                     & \(+\) Gaussian Noise     & 77.23 & 81.02 & 75.27   & 81.17    \\
%                     & \(+\) Projection         & 77.69 & 81.21 & 76.05   & 81.34    \\
%                     & \(+\) Ascend (Ours)      & 81.42 & 82.76 & 81.54   & 82.79    \\ \hline
% \multirow{4}{*}{75} & Baseline ($\lambda = 0$) & 76.27 & 84.71 & 38.94   & 76.27    \\
%                     & \(+\) Gaussian Noise     & 87.17 & 86.8  & 64.88   & 81.49    \\
%                     & \(+\) Projection         & 87.12 & 86.75 & 65.11   & 81.56    \\
%                     & \(+\) Ascend (Ours)      & 87.25 & 86.94 & 68.76   & 82.14    \\ \hline
% \end{tabular}
}
\end{sc}
\end{center}
\caption{Ablation study on the negative samples generation. The results are conducted on BANKING with known classes proportion 25\%, 50\% and 75\%. Baseline represents the experiment with no synthesized negative samples under the \ovr framework. }
\label{table:discussion_negative}
\end{table}

==> tabels/main_results.tex <==
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
%                       &          & \multicolumn{2}{c}{BANKING77}   & \multicolumn{2}{c}{CLINIC150}   & \multicolumn{2}{c}{StackOverflow}              \\ \midrule
% \multirow{8}{*}{25\%} & Methods  & Accuracy       & F1-score       & Accuracy       & F1-score       & Accuracy       & \multicolumn{1}{c|}{F1-score} \\ \cmidrule(l){2-8} 
%                       & MSP      & 43.67          & 50.09          & 47.02          & 47.62          & 28.67          & 37.85                         \\
%                       & DOC      & 56.99          & 58.03          & 74.97          & 66.37          & 42.74          & 47.73                         \\
%                       & OpenMax  & 49.94          & 54.14          & 68.50          & 61.99          & 40.28          & 45.98                         \\
%                       & DeepUnk  & 64.21          & 61.36          & 81.43          & 71.16          & 47.84          & 52.05                         \\
%                       & ADB      & 78.85          & 71.62          & 87.59          & 77.19          & 86.72          & \textbf{80.83}                \\
%                       & SelfSup* & 74.11          & 69.93          & 88.44          & 80.73          & 68.74          & 65.64                         \\
%                       & Ours     & \textbf{83.01} & \textbf{73.77} & \textbf{92.90} & \textbf{84.31} & \textbf{87.33} & \textbf{80.83}                \\ \midrule
% \multirow{7}{*}{50\%} & MSP      & 59.73          & 71.18          & 62.96          & 70.41          & 52.42          & 63.01                         \\
%                       & DOC      & 64.81          & 73.12          & 77.16          & 78.26          & 52.53          & 62.84                         \\
%                       & OpenMax  & 65.31          & 74.24          & 80.11          & 80.56          & 60.35          & 68.18                         \\
%                       & DeepUnk  & 72.73          & 77.53          & 83.35          & 82.16          & 58.98          & 68.01                         \\
%                       & ADB      & 78.86          & 80.90          & 86.54          & 85.05          & 86.40          & 85.83                         \\
%                       & SelfSup* & 72.69          & 79.21          & 88.33          & \textbf{86.67} & 75.08          & 78.55                         \\
%                       & Ours     & \textbf{81.07} & \textbf{81.72} & \textbf{88.49} & 86.50          & \textbf{86.84} & \textbf{86.12}                \\ \midrule
% \multirow{7}{*}{75\%} & MSP      & 75.89          & 83.60          & 74.07          & 82.38          & 72.17          & 77.95                         \\
%                       & DOC      & 76.77          & 83.34          & 78.73          & 83.59          & 68.91          & 75.06                         \\
%                       & OpenMax  & 77.45          & 84.07          & 76.80          & 73.16          & 74.42          & 79.78                         \\
%                       & DeepUnk  & 78.52          & 84.31          & 83.71          & 86.23          & 72.33          & 78.28                         \\
%                       & ADB      & 81.08          & \textbf{85.96} & 86.32          & 88.53          & 82.78          & 85.99                         \\
%                       & SelfSup* & 81.07          & 86.98          & \textbf{88.08} & \textbf{89.43} & 81.71          & 85.85                         \\
%                       & Ours     & \textbf{81.15} & 85.75          & \textbf{88.09} & 88.98          & \textbf{83.88} & \textbf{87.07}                \\ \bottomrule
% \end{tabular}
% \begin{table*}[h!]
% \begin{center}
% \begin{sc}
%   \scalebox{0.9}{
% \begin{tabular}{cccccccc}
% \hline
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{BANKING77}   & \multicolumn{2}{c}{CLINIC150}   & \multicolumn{2}{c}{StackOverflow} \\ \hline
% \%                   & Methods              & Accuracy       & F1-score       & Accuracy       & F1-score       & Accuracy        & F1-score        \\ \hline
% \multirow{7}{*}{25}  & MSP                  & 43.67          & 50.09          & 47.02          & 47.62          & 28.67           & 37.85           \\
%                      & DOC                  & 56.99          & 58.03          & 74.97          & 66.37          & 42.74           & 47.73           \\
%                      & OpenMax              & 49.94          & 54.14          & 68.5           & 61.99          & 40.28           & 45.98           \\
%                      & DeepUnk              & 64.21          & 61.36          & 81.43          & 71.16          & 47.84           & 52.05           \\
%                      & ADB                  & 78.85          & 71.62          & 87.59          & 77.19          & 86.72           & 80.83           \\
%                      & SelfSup*             & 74.11          & 69.93          & 88.44          & 80.73          & 68.74           & 65.64           \\
%                      & Ours                 & \textbf{80.11} & \textbf{73.35} & \textbf{92.64} & \textbf{84.81} & \textbf{90.14}  & \textbf{83.98}  \\ \hline
% \multirow{7}{*}{50}  & MSP                  & 59.73          & 71.18          & 62.96          & 70.41          & 52.42           & 63.01           \\
%                      & DOC                  & 64.81          & 73.12          & 77.16          & 78.26          & 52.53           & 62.84           \\
%                      & OpenMax              & 65.31          & 74.24          & 80.11          & 80.56          & 60.35           & 68.18           \\
%                      & DeepUnk              & 72.73          & 77.53          & 83.35          & 82.16          & 58.98           & 68.01           \\
%                      & ADB                  & 78.86          & 80.90           & 86.54          & 85.05          & \textbf{86.40}   & \textbf{85.83}  \\
%                      & SelfSup*             & 72.69          & 79.21          & 88.33          & 86.67          & 75.08           & 78.55           \\
%                      & Ours                 & \textbf{81.79} & \textbf{83.02} & \textbf{90.32} & \textbf{88.01} & 84.52           & 84.70           \\ \hline
% \multirow{7}{*}{75}  & MSP                  & 75.89          & 83.60           & 74.07          & 82.38          & 72.17           & 77.95           \\
%                      & DOC                  & 76.77          & 83.34          & 78.73          & 83.59          & 68.91           & 75.06           \\
%                      & OpenMax              & 77.45          & 84.07          & 76.80           & 73.16          & 74.42           & 79.78           \\
%                      & DeepUnk              & 78.52          & 84.31          & 83.71          & 86.23          & 72.33           & 78.28           \\
%                      & ADB                  & 81.08          & 85.96          & 86.32          & 88.53          & 82.78           & 85.99           \\
%                      & SelfSup*             & 81.07          & \textbf{86.98} & 88.08          & \textbf{89.43} & 81.71           & 85.85           \\
%                      & Ours                 & \textbf{82.16} & 86.68          & \textbf{88.36} & 89.16          & \textbf{83.33}  & \textbf{86.67}  \\ \hline
% \end{tabular}
% }
% \end{sc}
% \end{center}
% \caption{Results of open world classification on three datasets with different known class proportions. 
% % The scores of baseline methods are from the~\citep{zhang2021deep} and ~\citep{zhan2021out}.
% * means extra datasets are used during the training. \footnote{The first six baseline model results are from ~\citet{zhang2021deep}.
% The results of SelfSup are from the corresponding paper. }}
% \label{table:main}
% \end{table*}





% \begin{table*}[ht!]
% \begin{center}
% \begin{sc}
%   \scalebox{0.9}{
% \begin{tabular}{cccccccc}
% \hline
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{BANKING77}   & \multicolumn{2}{c}{CLINIC150}   & \multicolumn{2}{c}{StackOverflow} \\ \hline
% \%                   & Methods              & Accuracy       & F1-score       & Accuracy       & F1-score       & Accuracy        & F1-score        \\ \hline
% \multirow{7}{*}{25}  & MSP                  & 43.67          & 50.09          & 47.02          & 47.62          & 28.67           & 37.85           \\
%                      & DOC                  & 56.99          & 58.03          & 74.97          & 66.37          & 42.74           & 47.73           \\
%                      & OpenMax              & 49.94          & 54.14          & 68.5           & 61.99          & 40.28           & 45.98           \\
%                      & DeepUnk              & 64.21          & 61.36          & 81.43          & 71.16          & 47.84           & 52.05           \\
%                      & ADB                  & 78.85          & 71.62          & 87.59          & 77.19          & 86.72           & 80.83           \\
%                      & SelfSup*             & 74.11/-        & 69.93/-        & 88.44/81.96    & 80.73/71.15    & 68.74/-         & 65.64/-         \\
%                      & Ours                 & \textbf{80.27} & \textbf{73.42} & \textbf{92.64} & \textbf{84.81} & \textbf{90.14}  & \textbf{83.98}  \\ \hline
% \multirow{7}{*}{50}  & MSP                  & 59.73          & 71.18          & 62.96          & 70.41          & 52.42           & 63.01           \\
%                      & DOC                  & 64.81          & 73.12          & 77.16          & 78.26          & 52.53           & 62.84           \\
%                      & OpenMax              & 65.31          & 74.24          & 80.11          & 80.56          & 60.35           & 68.18           \\
%                      & DeepUnk              & 72.73          & 77.53          & 83.35          & 82.16          & 58.98           & 68.01           \\
%                      & ADB                  & 78.86          & 80.9           & 86.54          & 85.05          & \textbf{86.4}   & \textbf{85.83}  \\
%                      & SelfSup*             & 72.69/-        & 79.21/-        & 88.33/83.12    & 86.67/86.62    & 75.08/-         & 78.55/-         \\
%                      & Ours                 & \textbf{81.55} & \textbf{82.90} & \textbf{90.32} & \textbf{88.01} & 84.52           & 84.70           \\ \hline
% \multirow{7}{*}{75}  & MSP                  & 75.89          & 83.6           & 74.07          & 82.38          & 72.17           & 77.95           \\
%                      & DOC                  & 76.77          & 83.34          & 78.73          & 83.59          & 68.91           & 75.06           \\
%                      & OpenMax              & 77.45          & 84.07          & 76.8           & 73.16          & 74.42           & 79.78           \\
%                      & DeepUnk              & 78.52          & 84.31          & 83.71          & 86.23          & 72.33           & 78.28           \\
%                      & ADB                  & 81.08          & 85.96          & 86.32          & 88.53          & 82.78           & 85.99           \\
%                      & SelfSup*             & 81.07/-        & 86.98/-        & 88.08/84.16    & 89.43/86.90    & 81.71/-         & 85.85/-         \\
%                      & Ours                 & \textbf{82.45} & \textbf{87.06} & \textbf{88.36} & 89.16          & \textbf{83.33}  & \textbf{86.67}  \\ \cline{2-8} 
% \end{tabular}
% }
% \end{sc}
% \end{center}
% \caption{Results of open world classification on three datasets with different known class proportions. 
% % The scores of baseline methods are from the~\citep{zhang2021deep} and ~\citep{zhan2021out}.
% * means extra datasets are used during the training. \footnote{The baseline model results are from ~\citet{zhang2021deep}.}}
% \label{table:main}
% \end{table*}




% save 0623
% \begin{table*}[t]
% \begin{center}
% \begin{sc}
%   \scalebox{0.9}{
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% \multirow{2}{*}{\%} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{BANKING77}   & \multicolumn{2}{c}{CLINC}   & \multicolumn{2}{c}{StackOverflow} \\ \cmidrule(l){2-8} 
%                     & Methods              & Accuracy       & F1-score       & Accuracy       & F1-score       & Accuracy        & F1-score        \\ \midrule
% \multirow{7}{*}{25} & MSP                  & 43.67          & 50.09          & 47.02          & 47.62          & 28.67           & 37.85           \\
%                     & DOC                  & 56.99          & 58.03          & 74.97          & 66.37          & 42.74           & 47.73           \\
%                     & OpenMax              & 49.94          & 54.14          & 68.50          & 61.99          & 40.28           & 45.98           \\
%                     & DeepUnk              & 64.21          & 61.36          & 81.43          & 71.16          & 47.84           & 52.05           \\
%                     & ADB                  & 78.85          & 71.62          & 87.59          & 77.19          & 86.72           & 80.83           \\
%                     & SelfSup*             & 74.11          & 69.93          & 88.44          & 80.73          & 68.74           & 65.64           \\
%                     & Ours                 & \textbf{83.01} & \textbf{73.77} & \textbf{92.64} & \textbf{84.81} & \textbf{90.82}  & \textbf{83.63}  \\ \midrule
% \multirow{7}{*}{50} & MSP                  & 59.73          & 71.18          & 62.96          & 70.41          & 52.42           & 63.01           \\
%                     & DOC                  & 64.81          & 73.12          & 77.16          & 78.26          & 52.53           & 62.84           \\
%                     & OpenMax              & 65.31          & 74.24          & 80.11          & 80.56          & 60.35           & 68.18           \\
%                     & DeepUnk              & 72.73          & 77.53          & 83.35          & 82.16          & 58.98           & 68.01           \\
%                     & ADB                  & 78.86          & 80.90          & 86.54          & 85.05          & \textbf{86.40}  & \textbf{85.83}  \\
%                     & SelfSup*             & 72.69          & 79.21          & 88.33          & 86.67          & 75.08           & 78.55           \\
%                     & Ours                 & \textbf{81.07} & \textbf{81.72} & \textbf{90.23} & \textbf{88.01} & 85.79           & 85.74           \\ \midrule
% \multirow{7}{*}{75} & MSP                  & 75.89          & 83.60          & 74.07          & 82.38          & 72.17           & 77.95           \\
%                     & DOC                  & 76.77          & 83.34          & 78.73          & 83.59          & 68.91           & 75.06           \\
%                     & OpenMax              & 77.45          & 84.07          & 76.80          & 73.16          & 74.42           & 79.78           \\
%                     & DeepUnk              & 78.52          & 84.31          & 83.71          & 86.23          & 72.33           & 78.28           \\
%                     & ADB                  & 81.08          & 85.96          & 86.32          & 88.53          & 82.78           & 85.99           \\
%                     & SelfSup*             & 81.07          & \textbf{86.98} & 88.08          & 89.43          & 81.71           & 85.85           \\
%                     & Ours                 & \textbf{82.37} & 86.82          & \textbf{88.96} & \textbf{89.97} & \textbf{83.88}  & \textbf{87.07}  \\ \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{center}
% \caption{
% % \sj{the best system is marked wrong for Banking 77 at 75\%} 
% Results of open world classification on three datasets with different known class proportions. 
% % The scores of baseline methods are from the~\citep{zhang2021deep} and ~\citep{zhan2021out}.
% * indicates the use of extra datasets during the training. The first six results of the baseline model are from ~\citet{zhang2021deep}. The results for SelfSup are from the corresponding paper.
% % \footnotemark
% % \footnote{The first six baseline model results are from ~\citet{zhang2021deep}.
% % The results of SelfSup are from the corresponding paper. }
% }
% \label{table:main}
% \end{table*}
